Efficiency Requires Adaptation

The majority of historical designs are a priori in nature, where a priori indicates a design can be specified in advance of the experiment. The conventional wisdom is that the set of a priori designs is sufficient to produce efficient experiments. This work challenges this convention and finds that efficiency requires data dependent strategies. Specifically, in the context of a sequential experiment, where observations are accrued in a series of runs, an adaptive design is proposed that is guaranteed to be more efficient than any corresponding a priori design.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}

